Regularity and Continuity properties of the sub-Riemannian exponential map

We prove a version of Warner's regularity and continuity properties for the sub-Riemannian exponential map. The regularity property is established by considering sub-Riemannian Jacobi fields while the continuity property follows from studying the Maslov index of Jacobi curves. We finally show how this implies that the exponential map of the three dimensional Heisenberg group is not injective in any neighbourhood of a conjugate vector.

==> agrushin.tex <==
\section{Exponential map of the $\alpha$-Grushin plane}

\begin{theorem}
	\label{thm:geodesics}
	Let $\gamma : I \to \mathbb{G}_\alpha$ be horizontal path with initial value $\gamma(0) = (x_0, y_0)$ and initial covector $\lambda(0) = (u_0, v_0)$. In the case where $v_0 \neq 0$ and $(x_0, u_0) \neq 0$, the curve $\gamma$ is a geodesic if and only if
	\begin{equation}
		\label{geodesics}
		\left\{
		\begin{array}{rcl}
			x(t) & = & A \sin_\alpha(\omega t + \phi) \\
			y(t) & = & y_0 + v_0 \dfrac{A^{2 \alpha}}{(\alpha + 1)\omega^2}\left( \omega^2 t + \omega \cos_\alpha(\phi) \sin_\alpha(\phi) \right. \\
			& & \qquad \qquad \qquad \qquad \qquad \qquad \left. - \omega \cos_\alpha(\omega t + \phi) \sin_\alpha(\omega t + \phi) \right)\\
			u(t) & = & A \omega \cos_\alpha(\omega t + \phi) \\
			v(t) & = & v_0 \\
		\end{array}
		\right.
	\end{equation}
	for uniquely determined parameters $A > 0,\ \omega \in \mathbb{R} \setminus \{0\}$ and $\phi \in \left[0, 2 \pi_\alpha\right)$ satisfying
	\begin{equation}
		\label{basicrel}
		A^2 \omega^2 = u_0^2 + v_0^2 x_0^{2 \alpha}, \ \ \omega^2 = v_0^2 A^{2(\alpha - 1)}, \ \ x_0 = A \sin_\alpha(\phi) \text{ and } u_0 = A \omega \cos_\alpha(\phi).
	\end{equation}
	If $v_0 = 0$ or $(x_0, u_0) = 0$, the geodesic is $(x(t), y(t)) = (u_0 t + x_0, y_0)$ with its lift being constant: $(u(t), v(t)) = (u_0, v_0)$.
\end{theorem}

By simply differentiating the relations \cref{basicrel} with respect to $x_0, u_0$ and $v_0$, we find the following identities:
\begin{equation} 
	\label{derA}
	A_{x_0} = \dfrac{1 - \cos_\alpha^2(\phi)}{\sin_\alpha(\phi)} \text{,}\quad A_{u_0} = \dfrac{\cos_\alpha(\phi)}{\alpha \omega} \text{,}\quad A_{v_0} = \dfrac{-\cos^2_\alpha(\phi) A}{\alpha v_0};
\end{equation}
\begin{equation*}
	\omega_{x_0} = (\alpha - 1) \left( \dfrac{\omega}{A} \right) \left( \dfrac{1 - \cos_\alpha^2(\phi)}{\sin_\alpha(\phi)} \right) \text{,}\quad \omega_{u_0} = \left(\dfrac{\alpha - 1}{\alpha}\right) \dfrac{\cos_\alpha(\phi)}{\alpha A} \text{,}
\end{equation*}
\begin{equation}
	\label{derom}
	\omega_{v_0} = \dfrac{\omega}{v_0}\left(1 - \left(\dfrac{\alpha - 1}{\alpha}\right) \cos^2_\alpha(\phi) \right);
\end{equation}
\begin{equation}
	\label{derphi}
	\phi_{x_0} = \dfrac{\cos_\alpha(\phi)}{A}\text{,}\quad \phi_{u_0} = \dfrac{-\sin_\alpha(\phi)}{\alpha \omega A} \quad\text{ and}\quad \phi_{v_0} = \dfrac{\sin_\alpha(\phi)\cos_\alpha(\phi)}{\alpha v_0}.
\end{equation}

The symplectic moving frame $(E_1, E_2, F_1, F_2) = (\partial_u, \partial_v, \partial_x, \partial_y)$ along $\lambda(t)$ induced by the global coordinates of $\mathds{G}_\alpha$ satisfies \cref{movingframe}. The Jacobi fields along $\gamma$ are thus determined by the differential equation
\[
\begin{pmatrix}
	\dot{p} \\
	\dot{q}
\end{pmatrix}
=
\begin{pmatrix}
	- A(t)^T & R(t) \\
	B(t) & A(t)
\end{pmatrix}
\begin{pmatrix}
	p \\
	q
\end{pmatrix}.
\]

After some computations, we find that in the $\alpha$-Grushin plane, and for the chosen symplectic frame, the block matrices in the above differential equation are given by
\[
R(t) = 
\begin{pmatrix}
	- \alpha (2 \alpha - 1) v_0^2 x(t)^{2(\alpha - 1)} & 0\\
	0 & 0
\end{pmatrix},
\]
\[
A(t) = 
\begin{pmatrix}
	0 & 0 \\
	2 \alpha v_0 x(t)^{2\alpha - 1} & 0
\end{pmatrix}
\]
and the symmetric matrix
\[
B(t) = 
\begin{pmatrix}
	1 & 0 \\
	0 & x(t)^{2 \alpha}
\end{pmatrix}.
\]
ODE:
\[
\begin{pmatrix}
	\dot{p_1} \\
	\dot{p_2} \\
	\dot{q_1} \\
	\dot{q_2}
\end{pmatrix}
=
\begin{pmatrix}
	0 & - 2 \alpha v_0 x(t)^{2 \alpha - 1} & - \alpha (2 \alpha - 1) v_0^2 x(t)^{2(\alpha - 1)} & 0 \\
	0 & 0 & 0 & 0 \\
	1 & 0 & 0 & 0 \\
	0 & x(t)^{2 \alpha} & 2 \alpha v_0 x(t)^{2 \alpha - 1} & 0
\end{pmatrix}
\begin{pmatrix}
	p_1 \\
	p_2 \\
	q_1 \\
	q_2
\end{pmatrix}.
\]

\[
\ddot{q}_1(t) + \alpha (2 \alpha - 1) v_0^2 x(t)^{2(\alpha - 1)} q_1(t) = -2 \alpha v_0 x(t)^{2 \alpha - 1} p_2.
\]
$\dot{x}(t)$ is a solution of $\ddot{q}_1(t) + \alpha (2 \alpha - 1) v_0^2 x(t)^{2(\alpha - 1)} q_1(t) = 0$.
We are looking for a solution in terms of $x(t), y(t), \dot{x}(t), \dot{y}(t)$ (recall that they satisfy $\ddot{x} = - \alpha v_0^2 x^{2 \alpha - 1}$, $\dot{y} = v_0 x^{2 \alpha}$).
